On optimal ordering in the optimal stopping problem

In the classical optimal stopping problem, a player is given a sequence of random variables $X_1\ldots X_n$ with known distributions. After observing the realization of $X_i$, the player can either accept the observed reward from $X_i$ and stop, or reject the observed reward from $X_i$ and continue to observe the next variable $X_{i+1}$ in the sequence. Under any fixed ordering of the random variables, an optimal stopping policy, one that maximizes the player's expected reward, is given by the solution of a simple dynamic program. In this paper, we investigate the relatively less studied question of selecting the order in which the random variables should be observed so as to maximize the expected reward at the stopping time. To demonstrate the benefits of order selection, we prove a novel prophet inequality showing that, when the support of each random variable has size at most 2, the optimal ordering can achieve an expected reward that is within a factor of 1.25 of the expected hindsight maximum; this is an improvement over the corresponding factor of 2 for the worst-case ordering. We also provide a simple $O(n^2)$ algorithm for finding an optimal ordering in this case. Perhaps surprisingly, we demonstrate that a slightly more general case - each random variable $X_i$ is restricted to have 3-point support of form $\{0, m_i, 1\}$ - is NP-hard, and provide an FPTAS for that case.

==> FPTASolderProof.tex <==
\begin{proof}
	First define: $\Omega' = \{\sigma: V(X_{\sigma(n)})\geq \frac{\epsilon OPT}{2(n-1)}\}$, $\Omega'' = \{\sigma: V(X_{\sigma(n)})\geq \frac{\epsilon MAX^*}{2(n-1)}\}$, where $MAX^*$ is the value of $MAX$ (in Algorithm 2) at the end of the algorithm. Notice that since $MAX^*\leq OPT$, we have $\Omega'\subset\Omega''$. Let $OPT':= \max_{\sigma \in \Omega'} V_\sigma$, $OPT'':= \max_{\sigma \in \Omega''} V_\sigma$ and notice that $OPT'\leq OPT''$.
	
	We apply induction to prove the following:
	
	\begin{claim}
	Suppose $(S, T)$ is a partition of $\{X_1,\ldots, X_i\}$ that is in $\Omega''$. We will prove by induction that within ${\cal L}^i$, there exists some partition $(S', T')$ such that either 
	
	\begin{equation}\label{first-case}
	(1-\frac{\epsilon}{2n})^iV(T) \leq V(T')\leq V(T)
	\end{equation}
	
	or 
	
	\begin{equation}\label{second-case}
	(1-\frac{\epsilon}{2n})^iV(T') \leq V(T)\leq V(T')
	\end{equation}
	
	and $V(S', T')\geq (1-\frac{\epsilon}{2n})^iV(S, T)$.
	\end{claim}
	
    \begin{proof}	
	Suppose this is true for $i=k$. Assume $(S_{k+1}, T_{k+1})\in \Omega''$ is a partition of $\{X_1,\ldots, X_{k+1}\}$. Consider $S_k:= S_{k+1}\backslash X_{k+1}$, $T_k:=T_{k+1}\backslash X_{k+1}$. Then $(S_k, T_k)$ is a partition of $\{X_1,\ldots, X_k\}$.
	
	\xzcomment{This paragraph may not be fully rigorous yet, but should be clear.} If $T_k = \emptyset$, then it must be that $(S_k, \emptyset)\in {\cal L}^k$. Then, $(S_{k+1}, T_{k+1})$ must have been added into ${\cal L}^{k+1}$, but possibly trimmed. If it were trimmed, then there exists some $(S_{k+1}', T_{k+1}')$ where $V(S_{k+1}', T_{k+1}') \geq (1-\frac{\epsilon}{2n})V(S_{k+1}, T_{k+1})$ and satisfies either $(\ref{first-case})$ or $(\ref{second-case})$
	
	So assume that $T_k\neq \emptyset$. Then, $T_k$ and $T_{k+1}$ must share the same last random variable (since $X_{k+1}$ cannot be last because it has the largest conditional expectation thus far), hence $(S_k, T_k)\in \Omega''$. By induction, either equation $(\ref{first-case})$ or $(\ref{second-case})$ is true for $(S_k, T_k)$. Suppose that $(\ref{first-case})$ is true \xzcomment{I still need to do the other case, but it should be almost identical.} and the equation is satisfied by some pair $(S_k', T_k')\in L_k$. This means that $(1-\frac{\epsilon}{2n})^k V(T_k)\leq V(T_k')\leq V(T_k)$. This implies that $V(X_{k+1}, T_k')\leq V(X_{k+1}, T_k)$ and also
	
	\begin{eqnarray*}
	V(X_{k+1}, T_k')&=& V(X_{k+1}, V(T_k'))\\
	&\geq& V(X_{k+1}, (1-\frac{\epsilon}{2n})^kV(T_k))\\
	&\geq& (1-\frac{\epsilon}{2n})^k V(X_{k+1}, V(T_k)) 
	\end{eqnarray*}
	
	where the second line comes from the induction hypothesis and the third line comes from Lemma $\ref{lemma-3}$.
	Define:
	\[
    T_{k+1}' = \left\{\begin{array}{lr}
        T_k', & \text{if } X_{k+1}\in S_{k+1}\\
        T_k'\cup X_{k+1}, & \text{if } X_{k+1}\in T_{k+1}
        \end{array}\right\}
   \]
   
   	\[
    S_{k+1}' = \left\{\begin{array}{lr}
        S_k' \cup X_{k+1}, & \text{if } X_{k+1}\in S_{k+1}\\
        S_k'\cup X_{k+1}, & \text{if } X_{k+1}\in T_{k+1}
        \end{array}\right\}
   \]
   
    Then, the above result implies:
	
	$$(1-\frac{\epsilon}{2n})^kV(T_{k+1})\leq V(T_{k+1}')\leq V(T_{k+1})$$
	
	Now $(S_{k+1}', T_{k+1}')$ may not be in ${\cal L}^{k+1}$ since it may be removed in the Trim subroutine. However, if it is removed, there must be some $(S_{k+1}'', T_{k+1}'')$ where $V(T_{k+1}'')$ is in the same bucket as $V(T_{k+1}')$. We will prove that $(S_{k+1}'', T_{k+1}'')$ fulfills the inductive step. By the algorithm, if $V(T_{k+1}'')\leq V(T_{k+1}')$ then it must be that $(1-\frac{\epsilon}{2n})V(T_{k+1}')\leq V(T_{k+1}'')$. Then,
	
	\begin{eqnarray*}
	V(T_{k+1})&\geq& V(T_{k+1}'')\\
	&\geq& (1-\frac{\epsilon}{2n})V(T_{k+1}')\\
	&\geq& (1-\frac{\epsilon}{2n})^{k+1}V(T_{k+1})
	\end{eqnarray*}
	
	If instead $V(T_{k+1}')\leq V(T_{k+1}'')$, we have $(1-\frac{\epsilon}{2n})V(T_{k+1}'')\leq V(T_{k+1}')$. There are two cases: Either $V(T_{k+1}'')\leq V(T_{k+1})$ in which $(\ref{first-case})$ must hold. Otherwise, $V(T_{k+1}'')\geq V(T_{k+1})$. But since $(1-\frac{\epsilon}{2n})V(T_{k+1}'')\leq V(T_{k+1}')\leq V(T_{k+1})\leq V(T_{k+1}'')$, $(\ref{second-case})$ would hold. 
	
	Now we prove the second part of the induction:
	
	\begin{eqnarray*}
	V(S_{k+1}'', T_{k+1}'')&=& V(S_{k+1}'', V(T_{k+1}''))\\
	&\geq& V(S_{k+1}'', (1-\frac{\epsilon}{2n})V(T_{k+1}'))\\
	&\geq& (1-\frac{\epsilon}{2n})V(S_{k+1}'', T_{k+1}')\\
	&\geq& (1-\frac{\epsilon}{2n})V(S_{k+1}', T_{k+1}')\\
	&\geq& (1-\frac{\epsilon}{2n})^{k+1}V(S_{k+1}, T_{k+1})
	\end{eqnarray*}
	
	The second line is due to the size of the buckets in the Trim procedure. The third line is due to Lemma $\ref{lemma-3}$. The fourth line follows from Lemma $\ref{lemma-2}$. The last line is from the induction hypothesis. \sacomment{isn't induction hypothesis on $k$, not $k+1$?}

	\end{proof}
	
	Given the partition $(S, T)$ which realizes $OPT'$, the FPTAS returns a partition $(S'', T'')$ such that $V(S'', T'')\geq (1-\frac{\epsilon}{2n})^nOPT''\geq (1-\frac{\epsilon}{2n})^nOPT'$
\end{proof}

\begin{corollary}
	The FPTAS returns at least $(1-\epsilon)OPT$
\end{corollary}

\begin{proof}
	\begin{eqnarray*}
	ALG &\geq& (1-\frac{\epsilon}{2n})^nOPT'\\
	&\geq& (1-\frac{\epsilon}{2})OPT'\\
	&\geq& (1-\frac{\epsilon}{2})^2OPT\\
	&\geq& 1-\epsilon
	\end{eqnarray*}
	
	This follows from Proposition $\ref{ALG-OPT approx}$ and Lemma $\ref{Permutation-Subset}$.
\end{proof}


==> Preliminaries.tex <==
\section{Preliminaries}\label{Preliminaries}

Throughout this paper, we assume that all random variables are non-negative and independent. In addition, when we talk about an ordering $(X_1,\ldots, X_n)$, we mean that if $i<j$, then $X_i$ arrives before $X_j$.\\

The following definitions and lemma are from \cite{hill1983prophet} and \cite{hill1985selection}. We assume that all random variables are integrable throughout this paper.

\begin{definition}
	Let $X_i$ be a independent random variables and $(X_1,X_2,\ldots,X_n)$ be an ordering of those random variables. Then $V(X_1,\ldots, X_n) = \sup E[X_t]$ where the supremum is taken over all stopping rules for $X_1,\ldots,X_n$. 
\end{definition}

We allow $X_i$ to be degenerate random variables. For example, sometimes we will have an ordering $(X, c)$ where $c\in\mathbb{R}$. This merely means that first we observe $X$, and if we reject $X$, we are offered a reward of $c$. We will also frequently write $V(X, c)$ where $c$ is just treated as a degenerate random variable.

\begin{definition}
	Let the \textbf{worth} of random variables $\mathcal{X} = \{X_1,\ldots,X_n\}$, denoted as $W(X_1,\ldots,X_n)$ or $W(\mathcal{X})$, represent the optimal expected reward for a player free to choose the order of the random variables.
\end{definition}

\begin{lemma}\label{optimal_thresholds}
	Let $X_1,\ldots, X_n$ be independent random variables. Then
	\begin{enumerate}
		\item $V(X_j,\ldots, X_n) = E[\max\{X_j, V(X_{j+1},\ldots, X_n)\}]$ for $j=1\ldots n-1$
		\item if $t^*$ is the stop rule defined by $t^*=j \Leftrightarrow \{t^* > j-1 \text{ and } X_j\geq V(X_{j+1}, \ldots, X_n)\}$, then $E[X_{t^*}] = V(X_1,\ldots,X_n)$.
	\end{enumerate}
\end{lemma}

Lemma \ref{optimal_thresholds} states that when the ordering is fixed, the optimal stopping criteria to use is found by backward recursion. Therefore, the difficulty lies in finding the optimal ordering and not when to stop.\\

Here we prove a few useful lemmas that we will use throughout the paper.

\begin{lemma}\label{monotonicity}
	\textbf{Monotonicity:} Fix a random variable $X$. If $c_1\geq c_2$, then $V(X, c_1)\geq V(X, c_2)$.
\end{lemma}

\begin{proof}
	Suppose $c_1 \geq c_2$. It is easy to see that whatever stopping rule we use to attain $V(X, c_2)$ can also be used on the order $(X, c_1)$, and this policy will attain at least $V(X, c_2)$. Thus, $V(X, c_1)\geq V(X, c_2)$. 
\end{proof}

The following two lemmas are useful for simplifying random variables as it implies that both additive and multiplicative scaling does not change the optimal ordering.

\begin{lemma}\label{scaling}
	\textbf{Additive Scaling:} Let $X_1,\ldots X_n$ be non-negative random variables and let $c\in\mathbb{R}$ be a constant such that $Y_i:= X_i + c$ is still a non-negative random variable. Let $\sigma$ be a permutation. Then $V(Y_{\sigma(1)}, \ldots, Y_{\sigma(n)}) = V(X_{\sigma(1)}, \ldots, X_{\sigma(n)}) + c$.
\end{lemma}

\begin{proof}
	We prove by induction. For one variable, $V(Y) = E[Y] = E[X + c] = V(X) + c$.
	We denote for convenience $c':= V(X_{\sigma(2)}\ldots, X_{\sigma(k+1)})$. For the inductive step.
	
	\begin{eqnarray*}
	V(Y_{\sigma(1)},\ldots, Y_{\sigma(k+1)}) &=& V(Y_{\sigma(1)}, V(Y_{\sigma(2)}\ldots, Y_{\sigma(k+1)}))\\
	&=&V(X_{\sigma(1)} + c, V(X_{\sigma(2)}\ldots, X_{\sigma(k+1)}) + c)\\
	&=&V(X_{\sigma(1)} + c, c' + c)\\
	&=&P(X_{\sigma(1)} + c > c' + c)E[X_{\sigma(1)} + c|X_{\sigma(1)} + c > c' + c] +P(X_{\sigma(1)} + c \leq c' + c)(c' + c)\\
	&=& P(X_{\sigma(1)}> c')E[X_{\sigma(1)} + c|X_{\sigma(1)}> c'] +P(X_{\sigma(1)}\leq c')(c' + c)\\
	&=&	V(X_{\sigma(1)},\ldots, X_{\sigma(k+1)}) + c
	\end{eqnarray*}
\end{proof}

\begin{lemma}\label{Mult-Scaling}
	\textbf{Multiplicative Scaling:} Given non-negative random variables $X_1,\ldots, X_n$, define $Y_i:=\alpha X_i$ where $\alpha > 0$. Then if $\sigma$ is a permutation giving the optimal ordering for $X_1,\ldots, X_n$, then it also gives the optimal ordering for $Y_1, \ldots, Y_n$.
\end{lemma}

\begin{proof}
	\textcolor{red}{FINISH PROOF}
\end{proof}

Our main problem is the following:

\begin{problem}\label{secretary_ordering}
	Let $X:=\{X_1,\ldots, X_n\}$ be known, independent random variables. Let $\mathcal P_n$ be the set of permutations on $\{1,\ldots,n\}$. Then we wish to find $\max_{\sigma\in P_n} V(X_{\sigma(1)},\ldots,X_{\sigma(n)})$. 
\end{problem}

Our goal in this paper is to find cases when we can easily derive the optimal permutation of  $\{X_1,\ldots,X_n\}$ without resorting to a brute-force check of all permutations. 

==> Scheduling.tex <==
%\section{Scheduling Formulation}
\label{Scheduling}
In this section, we show an equivalency between Problem \ref{secretary_ordering} and a scheduling problem described in Problem \ref{scheduling_problem}.

\begin{problem}\label{scheduling_problem}
We are given a single machine $M$ and a set of $n$ jobs $\mathcal J=\{j_1,\ldots,j_n\}$, with corresponding processing times $p_j(t)$. $p_j(t)$ are decreasing convex functions of its starting time and such that $\lim_{t\to\infty} p_j(t) = 0$ and $\lim_{t\to 0^+} p_j'(t) \geq -1$. We wish to maximize the time to complete all jobs, i.e. its makespan $C_{max}$, subject to the machine not idling (the machine must be running a job at all times). We denote the optimal maximum makespan given $p_1,\ldots, p_n$ as $C_{max}(p_1,\ldots, p_n)$
\end{problem}

\begin{theorem}\label{scheduling_equivalency}
	There exists a bijection between $X_1,\ldots, X_n$ and a set of functions $p_1(t),\ldots, p_n(t)$ satisfying the conditions in Problem \ref{scheduling_problem} such that $W(X_1,\ldots, X_n) = C_{max}(p_1,\ldots, p_n)$
\end{theorem}
	
\begin{proof}
	Suppose we are given an instance of Problem $\ref{secretary_ordering}$, i.e. a set of secretaries $\{X_1,\ldots, X_n\}$. For $c>0$, define:
	
	\begin{eqnarray*}
	m_i(c) &:=& E[X_i|X_i\geq c] P(X_i\geq c) + cP(X_i < c)- c\\
	&=& E[X_i|X_i\geq c] - (1-P(X_i < c))c\\
	&=& P(X_i\geq c)(E[X_i|X_i\geq c] - c)\\
	&=& \int_c^\infty xdF_i - c\int_c^\infty dF_i\\
	&=& \int_c^\infty (x-c)dF_i
	\end{eqnarray*}
	
	Differentiating $m_i$, we get that 
	\begin{eqnarray*}
		m_i'(c) &=& -cf_i(c) - [-cf_i(c) + \int_c^\infty dF_i]\\
		&=&	-P(x_i\geq c)
	\end{eqnarray*}
	
	The second derivative is $m_i''(c) = f_i(x) > 0$, so $m_i(c)$ is a convex, decreasing function in $c$. For each $X_i$, we construct a job $j_i$ with processing time $p_i(t):= m_i(t)$. Notice that $\lim_{t\to\infty} p_i(t) = \lim_{t\to\infty} \int_t^\infty (x-t)dF_i = 0$, $p_i$ is a decreasing convex function, $\lim_{t\to 0^+}p_i'(t)\geq -1$, satisfying the conditions in Problem \ref{scheduling_problem}.\\
	
	Now suppose we are given an instance of Problem $\ref{scheduling_problem}$, that is, we are given a set of convex decreasing processing times $p_j(t)$ such that $\lim_{t\to\infty} p_j(t)= 0$, $\forall j$, $\lim_{t\to 0^+}p_j'(t)= -1$, and $p_j$ is continuous. Then define the random variable $X_j$ to have the cumulative distribution function $F_j(x) = (1+p_j'(x))$. Notice that $\lim_{x\to 0} F_j(x) = 0$ and $\lim_{x\to\infty} F_j(x) = \lim_{x\to\infty} 1+p_j'(x) = 1$. Furthermore, since $p_j(x)$ is convex, this implies that $p_j''(x)\geq 0$ and hence $F_j'(x) = f_j(x) = p_j''(x)\geq 0$, so $F_j$ is non-decreasing. This proves that $F_j(x)$ as defined is a distribution function.\\
	
	To finish the proof, we prove that $m_j(t)=p_j(t)$ for $X_j$ defined as having $F_j$ as distribution function.
	
	\begin{eqnarray*}
	m_j(t) &=& \int_{t}^\infty f_j(x)(x-t)dF_i\\
	&=&\int_{t}^\infty p_j''(x)(x-t)dx\\
	&=&\int_t^\infty xp_j''(x)dx - t\int_t^\infty p_j''(x)dx\\
	&=&-tp_j'(t)-\int_t^\infty p_j'(x)dx + tp_j'(t)\\
	&=&p_j(t)
	\end{eqnarray*}
	
	We now just have to prove that both instances attain the same optimal objective. Suppose the order $X_1,\ldots, X_n$ is the optimal secretary order which attains an objective value of $V(X_1,\ldots, X_n)$. Notice that $V(X_1,\ldots, X_n) = m_n(c_n) + m_{n-1}(c_{n-1}) + \ldots + m_1(c_1)$ where $c_n = 0$ and $c_i$ is defined recursively as $c_i:= m_n(c_n) + \ldots m_{i+1}(c_i)$ for $i<n$. By interpreting $m_i(c)$ as the processing time of $j_i$ at time $c$, we see that the quantity $V(X_1,\ldots, X_n)$ is precisely the makespan of the schedule under the ordering $j_n, j_{n-1}, \ldots, j_1$.
\end{proof}

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}


%\subsection{Other solvable cases}
\subsection{Optimal ordering for uniform distributions}
In this section, we will find the optimal ordering when the random variables $X_i$ form a nested sequence with support $[a_i, b_i]$. In \cite{hill1985selection}, it was shown that uniform random variables with support $[0, b_i]$ should be ordered by decreasing $b_i$, thus our result generalizes theirs. 

\begin{prop}
	Let $X_1,X_2,\ldots,X_n$ be uniform random variables such that $[a_j,  b_j]\subseteq [a_i, b_i]$ for $i<j$. Then the optimal ordering is $(X_1,X_2,X_3,\ldots,X_n)$. 
\end{prop}

\begin{proof}
	It is enough to show that for any two consecutive random variables $X_i$ and $X_{i+1}$ in an ordering, if $[a_{i+1}, b_{i+1}]\subseteq [a_i, b_i]$, it is always preferable to examine $X_i$ first and then $X_{i+1}$. Because of monotonicity (Lemma \ref{monotonicity}), it is sufficient to only consider the tail end of the ordering (i.e. either $(X_i, X_{i+1}, \ldots)$ or $(X_{i+1}, X_i, \ldots)$). Wlog, assume the two orderings under consideration are $(X_1, X_2, \ldots)$ or $(X_2, X_1, \ldots)$. That is, we fix the ordering after $X_1, X_2$ and suppose the expected reward for that part of the ordering is some real number $c\geq 0$. Thus, our problem is reduced to determining whether $(X_1, X_2, c)$ or $(X_2, X_1, c)$ offers a better expected reward.  
	
	Wlog, we scale $X_1$ and $X_2$ (using Lemmas \ref{scaling}, \ref{Mult-Scaling}) such that $X_1\sim U[0,1]$ and $X_2\sim U[a,b]$ where $0<a<b<1$. Let $ALG:S\to \R$ give the expected return under optimal thresholding, where $S = \{(X_1, X_2, c), (X_2, X_1, c)\}$. Let $ALG^+:S\to \R$ give the expected return under optimal thresholding, and which also receives the information $X_1\in [0,a]$, $X_1\in [a,b]$, or $X_1\in [b,1]$ in advance.
	
	Now, we make the observation that $ALG(X_1,X_2,c)\leq ALG^+(X_1,X_2,c)$ since we can simply ignore the additional information that $ALG^+$ provides and $ALG^+$ will return the same value as $ALG$. Hence, $\max\{ALG(X_1,X_2,c),ALG(X_2,X_1,c)\}\leq \max\{ALG^+(X_1,X_2,c),ALG^+(X_2,X_1,c)\}$.
	
	Furthermore, $ALG^+(X_2,X_1,c)= ALG^+(X_1,X_2,c)$. If $X_1\in [0,a]$, we will always reject $X_1$ regardless of whether it comes first or second. In this case, $ALG^+(X_2,X_1,c)=ALG^+(X_1,X_2,c)$. 
	If $X_1\in [a,b]$, then $X_1$ truncated at $[a,b]$ is distributed $U[a,b]$ so it is iid with $X_2$. In this case, the ordering does not matter, hence $ALG^+(X_2,X_1,c)=ALG^+(X_1,X_2,c)$.
	Finally, if $X_1\in [b,1]$, we will always reject $X_2$. Then, the ordering does not matter and $ALG^+(X_2,X_1,c)= ALG^+(X_1,X_2,c)$.
	
	Hence, $\max\{ALG^+(X_1,X_2,c),ALG^+(X_2,X_1,c)\}=ALG^+(X_1,X_2,c)$. Furthermore, $ALG^+(X_1,X_2,c)=ALG(X_1,X_2,c)$. This is because, since $X_1$ comes first, knowing the extra information in $ALG^+$ does not help. Therefore, we have the inequality
	
	\begin{eqnarray*}
	\max\{ALG(X_1,X_2,c),ALG(X_2,X_1,c)\}&\leq & \max\{ALG^+(X_1,X_2,c),ALG^+(X_2,X_1,c)\}\\
	&=& ALG^+(X_1,X_2,c)\\
	&=& ALG(X_1,X_2,c)
	\end{eqnarray*}
	
	Hence, it is always beneficial to order $X_1$ before $X_2$ regardless of the remaining sequence. This proves the result.
\end{proof}

%\begin{corollary}
%	\textcolor{red}{SCHEDULING EQUIVALENT VERSION OF PROPOSITION}
%\end{corollary}

%\subsection{Connections to scheduling problems}
%\input{Scheduling.tex}
